Notes on the Sigma invariants

Memoir on the Sigma invariants and their applications, version 2

==> Z.Definitions.tex <==
%
\makeatletter
%
%
\DeclareMathOperator{\ab}{ab}
\DeclareMathOperator{\add}{add}
\DeclareMathOperator{\Aff}{Aff}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\Aut}{Aut}
%   B
\DeclareMathOperator{\BPL}{BPL}
\DeclareMathOperator{\BS}{BS}

%   C
\DeclareMathOperator{\can}{can}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\core}{core}
%   D
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\defi}{def}
\DeclareMathOperator{\dis}{dis}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\Dr}{Dr}
%   E
\DeclareMathOperator{\e}{e}
\DeclareMathOperator{\edg}{E}
\DeclareMathOperator{\EG}{EG}
\DeclareMathOperator{\EL}{EL}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Ext}{Ext}
%   F
\DeclareMathOperator{\face}{face}
\DeclareMathOperator{\FF}{FF}
\DeclareMathOperator{\Fit}{Fit}
\DeclareMathOperator{\FP}{FP}
\DeclareMathOperator{\Frat}{Frat}
%   G

\DeclareMathOperator{\gp}{gp}
\DeclareMathOperator{\GL}{GL}
%   H
\DeclareMathOperator{\Cohom}{H}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Homeo}{Homeo}
%  I
\newcommand{\id}{\mathbbm{1}}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Inn}{Inn}
\DeclareMathOperator{\inv}{inv}
%   M
\DeclareMathOperator{\md}{md}
%  N
\newcommand{\norm}[1]{\| #1\|}
%  O
\DeclareMathOperator{\odd}{odd}
%  P
\DeclareMathOperator{\PD}{PD}
\DeclareMathOperator{\PL}{PL}
%  Q
\DeclareMathOperator{\Quot}{Quot}
%   R
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\rk}{rk}

%    S
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\sing}{sing}
\DeclareMathOperator{\myspan}{span}
\DeclareMathOperator{\stab}{St}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\SUPP}{SUPP}
\DeclareMathOperator{\sym}{sym}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\sgp}{sgp}
\DeclareMathOperator{\smd}{smd}
%  T
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\tor}{tor}
\DeclareMathOperator{\TPL}{TPL}
%   V
\DeclareMathOperator{\Val}{Val}
\DeclareMathOperator{\ver}{V}
%
%%
%%
\def\B{\mathbb{B}} 
\def\C{\mathbb{C}}
\def\E{\mathbb{E}}
\def\F{\mathbb{F}}
\def\G{\mathbb{G}}
\def\H{\mathbb{H}}
\def\I{\mathbb{I}}
\def\K{\mathbb{K}}
\def\L{\mathbb{L}}
\def\M{\mathbb{M}}
\def\N{\mathbb{N}}
\def\P{\mathbb{P}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\s{\mathbb{S}}
\def\U{\mathbb{U}}
\def\Z{\mathbb{Z}}
%
%
%% Calligraphic letters
\let\@@angstroem=\AA    
\let\angstroem=\@@angstroem
\def\AA{\mathcal{A}}
\def\BB{\mathcal{B}}
\def\CC{\mathcal{C}}
\def\DD{\mathcal{D}}
\def\EE{\mathcal{E}}
\def\FF{\mathcal{F}}
\def\GG{\mathcal{G}}
\def\HH{\mathcal{H}}
\def\II{\mathcal{I}}
\def\JJ{\mathcal{J}}
\def\KK{\mathcal{K}}
\def\LL{\mathcal{L}}
\def\MM{\mathcal{M}}
\def\NN{\mathcal{N}}
\def\OO{\mathcal{O}}
\def\PP{\mathcal{P}}
\def\QQ{\mathcal{Q}}
\def\RR{\mathcal{R}}
\def\SS{\mathcal{S}}
\def\TT{\mathcal{T}}
\def\UU{\mathcal{U}}
\def\VV{\mathcal{V}}
\def\WW{\mathcal{W}}
\def\XX{\mathcal{X}}
\def\YY{\mathcal{Y}}
\def\ZZ{\mathcal{Z}}
%%


%
%% Morphisms
%
\newcommand{\mono}{\rightarrowtail}
\newcommand{\incl}{\hookrightarrow}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\iso}{\stackrel{\sim}{\longrightarrow}}
\newcommand{\isoinv}{\stackrel{\sim}{\longleftarrow}}
% Useful abbreviations
\newcommand{\eg}{e.\;g.}
\newcommand{\ie}{i.\;e.}
\newcommand{\Ka}{K{\"a}hler}
%

%  Various commands
\newcommand{\qed}{\square}
\newcommand{\act}[3]{{}^{#1} \mspace{#2mu} #3}
%
%
\makeatother
\endinput

==> Z.Layout.tex <==
%%
\makeatletter
%
%
%======================
% Theoremlike environments
%======================
%
\theoremheaderfont{\rmfamily\scshape}
%
{\theorembodyfont{\itshape}
\newtheorem{thm}{Theorem}[section]
\newtheorem{prp}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{crl}[thm]{Corollary}
\newtheorem{addendum}[thm]{Addendum}
%
\newtheorem{algo}[thm]{Algorithm}
\newtheorem{problem}[thm]{Problem}
\newtheorem{conjecture}{Conjecture}
%
\newtheorem{thmNN}{Theorem}
\newtheorem{prpNN}{Proposition}
\newtheorem{problemNN}{Problem}
\newtheorem{questionBGH}{Question}
\newtheorem{conjectureNN}{Conjecture}
%
\newtheorem{thmNote}{Theorem}
\newtheorem{prpNote}[thmNote]{Proposition}
\newtheorem{problemNote}[thmNote]{Problem}
\newtheorem{conjectureNote}[thmNote]{Conjecture}
}
%
{\theorembodyfont{\upshape}
\newtheorem{definition}[thm]{Definition}
\newtheorem{definitions}[thm]{Definitions}
\newtheorem{example}[thm]{Example}
\newtheorem{examples}[thm]{Examples}
\newtheorem{remark}[thm]{Remark}
\newtheorem{remarks}[thm]{Remarks}
\newtheorem{note}[thm]{Note}
\newtheorem{notes}[thm]{Notes}
}
%% 


% Divisions
%----------------
\renewcommand{\thechapter}{\Alph{chapter}}
\renewcommand{\thesection}{\thechapter \arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesubsection\alph{subsubsection}}
%
\renewcommand{\thethm}{\thesection.\arabic{thm}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\thetable}{\arabic{section}.\arabic{table}} 
\renewcommand{\thefigure}{\arabic{section}.\arabic{figure}} 
\renewcommand{\thethmNN}{\thesectionNN.\arabic{thmNN}}
\renewcommand{\theprpNN}{\thesectionNN.\arabic{prpNN}}
\renewcommand{\thethmNote}{\thechapter\theendnote.\arabic{thmNote}}
\renewcommand{\thequestionBGH}{1.1}

%
% Counters            
%--------------
%
\newcounter{sectionNN}
\newcounter{endnote}

\newcounter{problem}
\counterwithin{equation}{section}
\counterwithin*{footnote}{chapter}
%
%
% Environment 'proof'
%----------------------------
%
\newenvironment{proof}%
{\removelastskip%
\vspace{12 pt plus1pt}
\noindent\textit{Proof.}}%
{\hfill $\square$\par \medskip}%
%%

% Environment 'Sketch of proof'
%----------------------------
%
\newenvironment{sketch-proof}%
{\removelastskip%
\vspace{12 pt plus1pt}
\noindent\textit{Sketch of proof.}}%
{\hfill $\square$\par \medskip}%
%%



%%
% Layout of the page
%------------------------------------
\setlength{\textwidth}{125mm}%
\setlength{\textheight}{190mm}%
\setlength{\oddsidemargin}{1.6cm}%
\setlength{\evensidemargin}{1.6cm}%
\setlength{\headheight}{12pt}%
\setlength{\headsep}{20pt}%
\setlength{\topmargin}{0mm}%
\setlength{\marginparwidth}{\evensidemargin}%
%
%
% Float parameters
%
\setcounter{totalnumber}{4}
\setcounter{totalnumber}{5}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.5}
\setlength{\floatsep}{6 pt plus 1pt minus 2 pt}
\setlength{\textfloatsep}{6pt plus 1pt minus2pt}%
\setlength{\intextsep}{6pt plus 1pt minus2pt}%
\renewcommand{\floatpagefraction}{0.8}
%
%=============
% Defining the page styles
%=============
%
%-----------------
% Definition of  fonts
%-----------------
\newcommand{\specialfont}{cmss} 
%
\newcommand{\titlingfontup}{\usefont{T1}{\specialfont}{bx}{n}}
\newcommand{\titlingfontit}{\usefont{T1}{\specialfont}{bx}{it}}
\newcommand{\headerfont}{\usefont{T1}{\specialfont}{m}{it}}
\newcommand{\pagefont}{\usefont{T1}{\specialfont}{m}{it}}
%
%---------------------
% pagestyle front
%--------------------
%

\makepagestyle{front}
\makeheadrule{front}{\textwidth}{\normalrulethickness}%
\makeoddhead{front}{\headerfont \footnotesize \rightmark}{}{\pagefont \footnotesize \thepage}%
\makeevenhead{front}{\pagefont\footnotesize\thepage}{}{\headerfont\footnotesize \leftmark}%
%
%-----------------------
% pagestyle - main
%-----------------------
%
\makepagestyle{main}
\renewcommand{\chaptermark}[1]{\markboth {#1}{}}%
\renewcommand{\sectionmark}[1]{\markright {#1}}%
%
%
\makeheadrule{main}{\textwidth}{\normalrulethickness}
%
\makeoddhead{main}%
{\headerfont \footnotesize \thesection\quad \rightmark}{}%
{\pagefont \footnotesize \thepage}%
%
\makeevenhead{main}{\pagefont\footnotesize\thepage}{}%
{\headerfont\footnotesize \chaptername\  \thechapter \ : \  \leftmark}%

%
\makeoddfoot{main}{}{}{\headerfont \footnotesize \version on the Sigma invariants}%
\makeevenfoot{main}{\headerfont \footnotesize  Notes}{}{}%
%
%
%-----------------------
% pagestyle - main
%-----------------------
%
\makepagestyle{main-plain}
\makeevenfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}
\makeoddfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}
%
\makepagestyle{main-empty}
\makeevenfoot{main-empty}{}{}{}
\makeoddfoot{main-empty}{}{}{}
%
%
%----------------------
% pagestyle  back
%----------------------
%
\makepagestyle{back}
\renewcommand{\chaptermark}[1]{\markboth {#1}{}}%
\renewcommand{\sectionmark}[1]{\markright {#1}{}}%

\makeheadrule{back}{\textwidth}{\normalrulethickness}
%
\makeoddhead{back}%
{\headerfont \footnotesize \rightmark}{}{\pagefont \footnotesize \thepage}%
%
\makeevenhead{back}%
{\pagefont\footnotesize\thepage}{}{\headerfont\footnotesize \leftmark}%
%
%
%===============
% Defining the chapter styles
%===============
%
\renewcommand{\chapnamefont}{\titlingfontup}
\renewcommand{\chapnumfont}{\chapnamefont}
\renewcommand{\chaptitlefont}{\titlingfontup}
%
%-----------------------------
%  chapterstyle  front
%-----------------------------
%
\makechapterstyle{front}{%
%
\setlength{\beforechapskip}{0pt}
\renewcommand{\printchaptername}{}%
\renewcommand{\printchapternum}{}%
\setlength{\midchapskip}{0pt}%
%
\renewcommand{\printchaptertitle}[1]{%
\hrule 
\vspace*{0.8\baselineskip}
\centering \titlingfontup \huge  ##1 \par 
\vspace*{0.5\baselineskip}
\hrule}
%
\setlength{\afterchapskip}{50pt}
}
%
%------------
%  chapterstyle -- main
%------------
%
\makechapterstyle{main}{%
%
\setlength{\beforechapskip}{0pt}
\renewcommand{\printchaptername}{}%
\renewcommand{\printchapternum}{}%
\setlength{\midchapskip}{0pt}%
%
\renewcommand{\printchaptertitle}[1]{%
\hrule 
\vspace*{0.7\baselineskip}
\centering \titlingfontup \huge \thechapter \quad  ##1 \par 
\vspace*{0.4\baselineskip}
\hrule}
%
\setlength{\afterchapskip}{50pt}
}
%
%---------------
% chapterstyle back1 (for Bibliography)
%--------------
%
\makechapterstyle{back1}{%
%
\setlength{\beforechapskip}{0pt}
\renewcommand{\printchaptername}{}%
\renewcommand{\printchapternum}{}%
\setlength{\midchapskip}{0pt}%
%
\renewcommand{\printchaptertitle}[1]{%
\hrule 
\vspace*{0.8\baselineskip}
\centering \titlingfontup \huge  ##1 \par 
\vspace*{0.4\baselineskip}
\hrule}
%
\setlength{\afterchapskip}{50pt}
}
%
%---------------
% chapterstyle back2 (for Index)
%--------------
%

\makechapterstyle{back2}{%
%
\setlength{\beforechapskip}{0pt}
\renewcommand{\printchaptername}{}%
\renewcommand{\printchapternum}{}%
\setlength{\midchapskip}{0pt}%
%
\renewcommand{\printchaptertitle}[1]{%
\hrule 
\vspace*{0.7\baselineskip}
\centering \titlingfontup \huge  ##1 \par 
\vspace*{0.5\baselineskip}
\hrule}
%
\setlength{\afterchapskip}{50pt}
}

%
%----------------------------------------
% Modifying Table of Contents
%---------------------------------------
%
\renewcommand\tableofcontents{%
    \if@twocolumn
      \@restonecoltrue\onecolumn
    \else
      \@restonecolfalse
    \fi
    \chapter*{\contentsname
    %----------
        \@mkboth{ \contentsname}{\contentsname}}%
    %----------
    \@starttoc{toc}%
    \if@restonecol\twocolumn\fi
    }
%
%-------------------------------------
% Modification of Bibliography
%------------------------------------
%
\renewenvironment{thebibliography}[1]{%
%
\chapter*{\titlingfontup\bibname}%
       %---------- \MakeUppercase removed
      \@mkboth{\bibname}{\bibname}%
       %-------
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}
%
%----------------------------
%Modification of Index
%---------------------------
\renewenvironment{theindex}
               {\if@twocolumn
                  \@restonecolfalse
                \else
                  \@restonecoltrue
                \fi
                \twocolumn[\@makeschapterhead{\indexname}]%
                %----------  \MakeUppercase removed
               \@mkboth{\indexname}{\indexname}%
                %----------
                \thispagestyle{plain}\parindent\z@
                \parskip\z@ \@plus .3\p@\relax
                \columnseprule \z@
                \columnsep 35\p@
                \let\item\@idxitem}
               {\if@restonecol\onecolumn\else\clearpage\fi}
%               
\renewcommand{\indexcolsep}{15pt}
%
%
%===============
%
%%  commands for sections
%
%================
%
%
\setsecheadstyle{%
\titlingfontup\fontsize{14.4}{17pt}\selectfont \raggedright}
%
\setsubsecheadstyle{%
\titlingfontup\fontsize{12}{14pt}\selectfont \raggedright}
%
\setsubsubsecheadstyle{%

\usefont{T1}{cmss}{m}{it}  \fontsize{11}{13pt}\selectfont \raggedright}

\setparaheadstyle{%
\usefont{T1}{lmr}{m}{it}  \fontsize{10}{12.0pt}\selectfont \raggedright}
%
%
%
% New skips
%----------------
\newcommand{\skiphalfaline}{\vspace{6pt plus 1pt}}
\newcommand{\skipaline}{\vspace{12pt plus 1pt}}
%

%% Initialisation
\setlength{\parindent}{0.5cm}
\setlength{\parskip}{0pt}
%
\makeatother
\endinput
